Extending Bayesian analysis of circular data to comparison of multiple groups

Circular data are data measured in angles and occur in a variety of scientific disciplines. Bayesian methods promise to allow for flexible analysis of circular data. Three existing MCMC methods (Gibbs, Metropolis-Hastings, and Rejection) for a single group of circular data were extended to be used in a between-subjects design, providing a novel procedure to compare groups of circular data. Investigating the performance of the methods by simulation study, all methods were found to overestimate the concentration parameter of the posterior, while coverage was reasonable. The rejection sampler performed best. In future research, the MCMC method may be extended to include covariates, or a within-subjects design.

==> j1table.tex <==
% latex table generated in R 3.0.2 by xtable 1.7-1 package
% Mon May 12 00:53:49 2014
{\footnotesize
\begin{tabular}{ccccccccc}
  \toprule 
 &&& \multicolumn{2}{c}{Posterior $\mu$} & \multicolumn{2}{c}{Posterior $\kappa$ \footnote{Posterior $\kappa$ mode denotes the mode as described in section \ref{hdimode}. Coverage denotes the proportion of replications in which the true $\kappa$ fell within the 95 \% HDI.} }&  \\
   n & $\kappa$ & Method & Mean & Coverage & Mode & Coverage
                                            & Acc. \footnote{Acceptance ratio. For Gibbs sampling, this is always 1. For Metropolis-Hastings, $Q_{acc}/Q$ is given. For the rejection method, this is $Q/Q_{can}$.} & MCT \footnote{Mean Computation Time of one replication in seconds.} \\
 \midrule 
 5 & 0.1 & Gibbs & 28.51 & 0.78 & 0.67 & 0.96 & 1 & 0.78 \\ 
   &  & MH & 28.34 & 0.78 & 0.63 & 0.96 & 0.33 & 0.04 \\ 
   \vspace{0.2cm} &  & Rejection & 27.89 & 0.77 & 0.64 & 0.97 & 0.96 & 0.03 \\ 
   & 4 & Gibbs & 19.04 & 0.94 & 5.11 & 0.96 & 1 & 7.60 \\ 
   &  & MH & 19.01 & 0.90 & 9.83 & 0.93 & 0.63 & 0.04 \\ 
   \vspace{0.2cm} &  & Rejection & 19.02 & 0.91 & 7.65 & 0.95 & 1 & 0.04 \\ 
   & 32 & Gibbs & --- & --- & --- & --- & --- & --- \\ 
   &  & MH & 20.07 & 0.80 & 133.12 & 0.64 & 0.55 & 0.05 \\ 
   &  & Rejection & 20.07 & 0.88 & 55.74 & 0.96 & 1 & 0.05 \\ 
   \cmidrule{1-9}30 & 0.1 & Gibbs & 28.14 & 0.87 & 0.19 & 0.97 & 1 & 1.13 \\ 
   &  & MH & 28.68 & 0.88 & 0.18 & 0.97 & 0.16 & 0.07 \\ 
   \vspace{0.2cm} &  & Rejection & 28.50 & 0.86 & 0.19 & 0.98 & 0.98 & 0.04 \\ 
   & 4 & Gibbs & 19.96 & 0.94 & 4.25 & 0.92 & 1 & 9.91 \\ 
   &  & MH & 19.96 & 0.94 & 4.26 & 0.94 & 0.36 & 0.08 \\ 
   \vspace{0.2cm} &  & Rejection & 19.96 & 0.94 & 4.17 & 0.96 & 1 & 0.04 \\ 
   & 32 & Gibbs & --- & --- & --- & --- & --- & --- \\ 
   &  & MH & 20.04 & 0.93 & 34.71 & 0.95 & 0.71 & 0.08 \\ 
   &  & Rejection & 20.05 & 0.93 & 34.66 & 0.95 & 1 & 0.04 \\ 
   \cmidrule{1-9}100 & 0.1 & Gibbs & 19.50 & 0.92 & 0.12 & 0.98 & 1 & 3.94 \\ 
   &  & MH & 19.76 & 0.92 & 0.11 & 0.98 & 0.10 & 0.17 \\ 
   \vspace{0.2cm} &  & Rejection & 19.57 & 0.92 & 0.12 & 0.98 & 0.98 & 0.03 \\ 
   & 4 & Gibbs & 20.02 & 0.95 & 4.10 & 0.94 & 1 & 59.03 \\ 
   &  & MH & 20.02 & 0.95 & 4.11 & 0.95 & 0.21 & 0.17 \\ 
   \vspace{0.2cm} &  & Rejection & 20.02 & 0.95 & 4.04 & 0.96 & 1 & 0.03 \\ 
   & 32 & Gibbs & --- & --- & --- & --- & --- & --- \\ 
   &  & MH & 19.97 & 0.95 & 32.87 & 0.92 & 0.53 & 0.16 \\ 
   &  & Rejection & 19.97 & 0.95 & 32.81 & 0.92 & 1 & 0.04 \\ 
   \bottomrule 
\end{tabular}
}


==> j3table.tex <==
% latex table generated in R 3.0.2 by xtable 1.7-1 package
% Mon May 12 00:53:49 2014
{\footnotesize
\begin{tabular}{ccccccccccc}
  \toprule 
 &&& \multicolumn{4}{c}{Posterior $\mu$} & \multicolumn{2}{c}{Posterior $\kappa$ \footnote{Posterior $\kappa$ mode denotes the mode as described in section \ref{hdimode}. Coverage denotes the proportion of replications in which the true $\kappa$ fell within the 95 \% HDI.} }&  \\
   $n_j$ & $\kappa$ & Method & $\mu_1$ & $\mu_2$ & $\mu_3$ & Coverage & Mode & Coverage & Acc. \footnote{Acceptance ratio. For Gibbs sampling, this is always 1. For Metropolis-Hastings, $Q_{acc}/Q$ is given. For the rejection method, this is $Q/Q_{can}$.} & MCT \footnote{Mean Computation Time of one replication in seconds.} \\
 \midrule 
 5 & 0.1 & Gibbs & 21.97 & 52.40 & 64.60 & 0.52 & 0.79 & 0.75 & 1 & 1.18 \\ 
   &  & MH & 23.40 & 52.67 & 64.07 & 0.85 & 0.36 & 0.96 & 0.22 & 0.11 \\ 
   \vspace{0.2cm} &  & Rejection & 23.23 & 52.39 & 63.80 & 0.85 & 0.40 & 0.97 & 0.98 & 0.05 \\ 
   & 4 & Gibbs & 20.94 & 39.34 & 59.95 & 0.69 & 5.39 & 0.89 & 1 & 20.13 \\ 
   &  & MH & 20.95 & 39.33 & 59.96 & 0.94 & 4.69 & 0.96 & 0.47 & 0.13 \\ 
   \vspace{0.2cm} &  & Rejection & 20.95 & 39.34 & 59.96 & 0.94 & 4.57 & 0.97 & 1 & 0.06 \\ 
   & 32 & Gibbs & --- & --- & --- & --- & --- & --- & --- & --- \\ 
   &  & MH & 19.97 & 39.80 & 59.97 & 0.92 & 45.82 & 0.93 & 0.76 & 0.14 \\ 
   &  & Rejection & 19.97 & 39.80 & 59.97 & 0.92 & 38.37 & 0.95 & 1 & 0.06 \\ 
   \cmidrule{1-11} 
 30 & 0.1 & Gibbs & 32.41 & 33.81 & 61.85 & 0.60 & 0.30 & 0.85 & 1 & 1.19 \\ 
   &  & MH & 32.88 & 33.56 & 61.16 & 0.91 & 0.14 & 0.98 & 0.11 & 0.23 \\ 
   \vspace{0.2cm} &  & Rejection & 32.66 & 33.59 & 61.24 & 0.90 & 0.16 & 0.98 & 0.98 & 0.09 \\ 
   & 4 & Gibbs & 20.10 & 39.95 & 60.27 & 0.73 & 4.19 & 0.93 & 1 & 20.25 \\ 
   &  & MH & 20.10 & 39.95 & 60.27 & 0.95 & 4.12 & 0.96 & 0.22 & 0.24 \\ 
   \vspace{0.2cm} &  & Rejection & 20.10 & 39.95 & 60.27 & 0.95 & 4.04 & 0.97 & 1 & 0.14 \\ 
   & 32 & Gibbs & --- & --- & --- & --- & --- & --- & --- & --- \\ 
   &  & MH & 19.94 & 40.05 & 60.07 & 0.94 & 32.62 & 0.96 & 0.55 & 0.24 \\ 
   &  & Rejection & 19.94 & 40.05 & 60.07 & 0.94 & 32.59 & 0.95 & 1 & 0.18 \\ 
   \cmidrule{1-11} 
 100 & 0.1 & Gibbs & 19.50 & 44.97 & 58.58 & 0.67 & 0.18 & 0.91 & 1 & 3.75 \\ 
   &  & MH & 18.82 & 45.31 & 58.30 & 0.94 & 0.10 & 0.97 & 0.07 & 0.51 \\ 
   \vspace{0.2cm} &  & Rejection & 19.09 & 45.21 & 58.57 & 0.94 & 0.10 & 0.98 & 0.98 & 0.09 \\ 
   & 4 & Gibbs & 19.93 & 40.01 & 60.04 & 0.74 & 4.05 & 0.94 & 1 & 99.10 \\ 
   &  & MH & 19.93 & 40 & 60.04 & 0.95 & 4.03 & 0.95 & 0.13 & 0.52 \\ 
   \vspace{0.2cm} &  & Rejection & 19.93 & 40.01 & 60.04 & 0.95 & 3.97 & 0.96 & 1 & 0.10 \\ 
   & 32 & Gibbs & --- & --- & --- & --- & --- & --- & --- & --- \\ 
   &  & MH & 20.02 & 39.99 & 59.99 & 0.95 & 32.18 & 0.95 & 0.36 & 0.52 \\ 
   &  & Rejection & 20.02 & 39.99 & 59.99 & 0.95 & 32.19 & 0.96 & 1 & 0.08 \\ 
   \bottomrule 
\end{tabular}
}

